Kinship Verification Using Voice

Kinship verification (KV) from voice, the task of determining whether two speakers are biologically related, has received only little attention. Our work establishes a foundational basis for this emerging frontier, contributing to both performance evaluation and detection methodologies. First, leveraging the speech recordings of the large-scale audio-visual dataset, KAN-AV, we propose a revised evaluation protocol that controls for various confounders and adopts a family-disjoint train--test split to address open-set KV. Second, we analyze the close connection between speaker verification and KV, showing that genealogical similarity of speaker pairs plays opposite roles in the two tasks. Third, we tackle KV using three neural speaker embedding extractors (ECAPA-TDNN, WavLM-ECAPA, and ReDimNet) combined with various back-ends. In zero-shot KV including same-speaker target trials, ReDimNet achieves the lowest equal error rate (EER) of $20.8\%$; however, performance degrades to $39.7\%$ under strict kin trials, where same-speaker target trials are excluded. Our best trainable back-end, which applies asymmetric processing of the embedding pair to mitigate age-difference effects, obtains an EER of $32.0\%$ ($18.6\%$ with speaker target trials included). These results highlight the difficulty of KV while showing that speaker embeddings encode familial cues, offering a promising foundation for voice-based kinship analysis.

==> Methods.tex <==

\section{Kinship Verification using Speaker Embeddings}\label{sec:kinship-verification}
%To perform kinship verification, we considered two widely used speaker embeddings (1) ECAPA-TDNN~\cite{} and (2) RedimNet~\cite{}. 


Speaker embeddings~\cite{wang2024overview,desplanques2020ecapa} capture both physiological characteristics (e.g., vocal tract length and pitch) and behavioral–linguistic traits of individuals. Since each person is trivially a relative of oneself, we hypothesize that speaker embeddings also encode cues relevant to kinship. %and systematically evaluate their effectiveness for kin verification. 
In our systematic evaluation, we employ 
two complementary evaluation paradigms: (1) a zero-shot approach, in which we directly compute cosine similarity between embeddings to measure pairwise kin similarity, and (2) a trainable backend utilizing %in which we learn family-specific transformations using 
a Siamese network architecture~\cite{kefalas2023kan}. %Through this framework, we 
This allows us to assess
systematically, the extent to which speaker embeddings encode familial similarity and establish a scalable pipeline for kinship verification in both zero-shot and supervised settings.

\subsection{Cosine Similarity}

Given a trial pair with embeddings ${\bf e}_1, {\bf e}_2 \in \mathbb{R}^d$, we compute their cosine similarity as
\begin{equation}
s({\bf e}_1, {\bf e}_2) = \frac{{\bf e}_1^\top {\bf e}_2}{\|{\bf e}_1\|_2 \, \|{\bf e}_2\|_2},
\end{equation}
where $^\top$ and $\|\cdot\|_2$ denote transpose and 2-norm, respectively. We use the cosine score to detect the kin-target and kin non-target trials, with the usual ordering convention of higher score values indicating positive (kin) relation.


\subsection{Trainable Backends}

In the trainable setting, we consider three network designs, the first two of which follow a symmetric Siamese structure. First, we implement a \emph{fully connected} architecture inspired by TripletNet-based kinship recognition methods~\cite{kefalas2023kan}. Second, given the limited number of available training trials~\cite{barz2020deep}, we employ a simple \emph{affine cosine backend} that applies a shared affine transformation to both embeddings before cosine scoring. The model is trained under a constrained objective that regularizes the transformation toward the identity, thereby preserving the cosine geometry and speaker-discriminative structure of the original embedding space while adapting it to kinship verification. Third, to address the age and gender mismatches inherent in kinship verification, we introduce an asymmetric \emph{single-embedding affine projection} in which only one embedding is transformed while the other remains fixed.




\subsubsection{Fully Connected Network (FCN)}

Inspired by the kinship recognition study in~\cite{kefalas2023kan}, we implement a three-layer fully connected neural network. The network takes as input a speaker embedding of dimension $d$ and maps it to a lower-dimensional representation through two hidden layers of size $d/2$. Each linear transformation is followed by batch normalization and a nonlinear activation function to improve training stability and generalization. The transformation is defined as
\begin{equation}
\begin{aligned}
{\bf z}_i = f_\theta({\bf e}_i) 
= \phi_3\Big(&\mathrm{BN}_3\big({\bf W}_3 \,
\phi_2(\mathrm{BN}_2({\bf W}_2 \, \\
&\phi_1(\mathrm{BN}_1({\bf W}_1 {\bf e}_i + {\bf b}_1)) + {\bf b}_2))
+ {\bf b}_3\big)\Big),
\end{aligned}
\end{equation}
where $i \in \{1,2\}$ indexes the two embeddings in a trial pair, ${\bf W}_k$ and ${\bf b}_k$ denote the weight matrices and bias vectors, respectively, $\mathrm{BN}_k(\cdot)$ denotes batch normalization, and $\phi_k(\cdot)$ denotes a nonlinear activation function. In our experiments, we use the rectified linear unit (ReLU) as the activation function for all layers, i.e., for $k \in \{1,2,3\}$.


The network parameters are optimized using contrastive loss~\cite{hadsell2006dimensionality}, which encourages embeddings from kin-target pairs to be close in the transformed space while pushing embeddings from kin non-target pairs farther apart. The loss is defined as
\begin{equation}
\mathcal{L}_{c}
= y \, \|{\bf z}_1 - {\bf z}_2\|_2^2
+ (1-y)\,\max\!\left(0, m - \|{\bf z}_1 - {\bf z}_2\|_2\right)^2,
\end{equation}
where $y \in \{0,1\}$ indicates whether the pair is a kin target pair ($y=1$) or a kin non-target pair ($y=0$), and $m$ denotes the margin parameter.

Further, following~\cite{kefalas2023kan}, we regularize the learned representations by adding an $L_2$ penalty on the transformed embeddings during training. The overall training objective is
\begin{equation}
\mathcal{L}
= \mathcal{L}_{c}
+ \lambda_f \sum_{i=1}^{2} \|f_\theta({\bf e}_i)\|_2^2,
\end{equation}
where $\lambda_f$ controls the strength of the regularization.

% \begin{equation}
% s({\bf e}_1, {\bf e}_2) = \frac{{\bf z}_1^\top {\bf z}_2}{\|{\bf z}_1\|_2 \, \|{\bf z}_2\|_2}.
% \end{equation}

\subsubsection{Affine Cosine Backend}
This backend is designed to provide a lightweight trainable adaptation~\cite{barz2020deep} of pretrained speaker embeddings for kinship verification while preserving the structure of the original embedding space. To this end, we apply the same \emph{affine transformation} to both embeddings in a trial and perform verification using cosine similarity in the transformed space. To avoid distorting the geometry of the original speaker embeddings, the transformation is regularized toward the identity mapping.

Formally, each input embedding is transformed as
\begin{equation}
{\bf z}_i = f_\theta({\bf e}_i) = {\bf W}{\bf e}_i + {\bf b},
\end{equation}
where ${\bf W} \in \mathbb{R}^{d \times d}$ is a linear transformation matrix and ${\bf b} \in \mathbb{R}^{d}$ is a bias vector. The transformed embeddings are subsequently length-normalized and compared using cosine scoring.


We optimize ${\bf W}$ and ${\bf b}$ using the combined objective
\begin{equation}
\mathcal{L} = \mathcal{L}_{\rm cosine} + \mathcal{L}_{\rm reg}.
\end{equation}
To preserve the structure of the original embedding space, we regularize the affine transformation toward the identity mapping:
\begin{equation}
\mathcal{L}_{\rm reg} = \lambda_w \|{\bf W} - {\bf I}\|_F^2 + \lambda_b \|{\bf b}\|_2^2,
\end{equation}
where ${\bf I}$ denotes the identity matrix and $\lambda_w$ and $\lambda_b$ are regularization coefficients. The cosine embedding loss is defined as
\begin{equation}
\mathcal{L}_{\rm cosine} =
\frac{1}{N} \sum_{i=1}^N
\begin{cases}
1 - s({\bf z}_1^{(i)}, {\bf z}_2^{(i)}), & y_i = 1, \\
\max\!\left(0, s({\bf z}_1^{(i)}, {\bf z}_2^{(i)}) - m\right), & y_i = -1,
\end{cases}
\end{equation}
where $y_i \in \{1,-1\}$ denotes the kin-target and kin non-target labels, respectively, and $m$ is the margin parameter.


\subsubsection{Single-Embedding Affine Projection}

To account for the asymmetric age- and gender-related variation that can arise in kinship verification, we consider a \emph{single-embedding affine projection} in which only one embedding in a trial is transformed, while the other is kept fixed. Because this formulation is directional, we first impose a deterministic ordering of the two embeddings within each trial during training so that the mapping is well defined.

Specifically, each embedding pair is reordered according to predefined criteria before being passed to the model. For age-constrained projection, the embedding of the older speaker is assigned to ${\bf e}_1$ and that of the younger speaker to ${\bf e}_2$. For gender-constrained projection, the male embedding is assigned to ${\bf e}_1$ in cross-gender trials. For joint age-and-gender-constrained projection, we first apply the age-based ordering and then enforce the gender-based rule within cross-gender pairs. This deterministic ordering removes directional ambiguity and encourages the model to learn systematic kin-related transformations associated with age and/or gender.

Formally, given an ordered trial pair ${\bf e}_1, {\bf e}_2 \in \mathbb{R}^{d}$, we define
\begin{equation}
{\bf z}_1 = f_\theta({\bf e}_1) = {\bf W}{\bf e}_1 + {\bf b},
\qquad
{\bf z}_2 = {\bf e}_2,
\end{equation}
where ${\bf W} \in \mathbb{R}^{d \times d}$ is a linear transformation matrix and ${\bf b} \in \mathbb{R}^{d}$ is a bias vector. The transformed and fixed embeddings are subsequently length-normalized and compared using cosine scoring. The parameters ${\bf W}$ and ${\bf b}$ are optimized using the same cosine embedding loss $\mathcal{L}_{\rm cosine}$ and identity regularization term $\mathcal{L}_{\rm reg}$ as in the affine cosine backend.
